Interventional Few-Shot Learning

We uncover an ever-overlooked deficiency in the prevailing Few-Shot Learning (FSL) methods: the pre-trained knowledge is indeed a confounder that limits the performance. This finding is rooted from our causal assumption: a Structural Causal Model (SCM) for the causalities among the pre-trained knowledge, sample features, and labels. Thanks to it, we propose a novel FSL paradigm: Interventional Few-Shot Learning (IFSL). Specifically, we develop three effective IFSL algorithmic implementations based on the backdoor adjustment, which is essentially a causal intervention towards the SCM of many-shot learning: the upper-bound of FSL in a causal view. It is worth noting that the contribution of IFSL is orthogonal to existing fine-tuning and meta-learning based FSL methods, hence IFSL can improve all of them, achieving a new 1-/5-shot state-of-the-art on \textit{mini}ImageNet, \textit{tiered}ImageNet, and cross-domain CUB. Code is released at https://github.com/yue-zhongqi/ifsl.

==> tables/comparison.tex <==
\begin{tabular}{c c@{\hskip6pt} c@{\hskip6pt} c@{\hskip6pt}}
    \toprule
    
    \textbf{Method} & \textbf{n-shot} &\textbf{Metric} & \textbf{Result}\\
    \midrule
    
    \multicolumn{1}{c}{\multirow{4}{*}{IFSL+kNN}} & \multicolumn{1}{c}{\multirow{2}{*}{5-shot}} & Acc & 78.54\\
    & & dAcc & 70.54\\
    & \multicolumn{1}{c}{\multirow{2}{*}{1-shot}} & Acc & 78.54\\
    & & dAcc & 70.54\\
    \midrule
    
    \multicolumn{1}{c}{\multirow{4}{*}{IdeMe-Net}} & \multicolumn{1}{c}{\multirow{2}{*}{5-shot}} & Acc & 78.54\\
    & & dAcc & 70.54\\
    & \multicolumn{1}{c}{\multirow{2}{*}{1-shot}} & Acc & 78.54\\
    & & dAcc & 70.54\\
    \bottomrule
\end{tabular}


==> tables/main_results_cells_v0.tex <==
\begin{tabular}{@{\hskip1pt}c @{\hskip1pt} c g g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g@{\hskip6pt} g{\hskip6pt}}
    \toprule
    \rowcolor{white}
    & & & \multicolumn{8}{c}{\textbf{ResNet-10}} & \multicolumn{8}{c}{\textbf{WRN-28-10}} \\
    
    \rowcolor{white}
    & & & \multicolumn{4}{c}{\textit{mini}ImageNet} & \multicolumn{4}{c}{\textit{tiered}ImageNet} & \multicolumn{4}{c}{\textit{mini}ImageNet} & \multicolumn{4}{c}{\textit{tiered}ImageNet} \\\cmidrule(l){4-7} \cmidrule(l){8-11} \cmidrule(l){12-15} \cmidrule(l){16-19}
    
    \rowcolor{white}
    & & & \multicolumn{2}{c}{$5$-shot} & \multicolumn{2}{c}{$1$-shot} & \multicolumn{2}{c}{$5$-shot} & \multicolumn{2}{c}{$1$-shot} & \multicolumn{2}{c}{$5$-shot} & \multicolumn{2}{c}{$1$-shot} & \multicolumn{2}{c}{$5$-shot} & \multicolumn{2}{c}{$1$-shot}\\
    
    \rowcolor{white}
    \multicolumn{3}{c}{\multirow{-4}{*}[0.5em]{\textbf{Method}}} & Acc & dAcc & Acc & dAcc & Acc & dAcc & Acc & dAcc & Acc & dAcc & Acc & dAcc & Acc & dAcc & Acc & dAcc\\
    \midrule
    
    
    \rowcolor{white}
     & \multicolumn{1}{c}{\multirow{2}{*}{\shortstack{Linear}}} & & 76.38 & 73.75 & 56.26 & 52.25 & 81.01 & 78.10 & 61.39 & 57.77 & 79.79 & 76.70 & 60.69 & 55.86 & 85.37 & 82.53 & 67.27 & 63.11\\
    & & IFSL & 77.97 & 75.62 & 60.13 & 56.40 & 82.08 & 79.58 & 64.29 & 60.97 & 80.97 & 78.13 & 64.12 & 59.64 & 86.19 & 84.00 & 69.96 & 67.05\\

    \rowcolor{white}
    &\multicolumn{1}{c}{\multirow{2}{*}{\shortstack{Cosine}}} & & 75.21 & 72.49 & 52.35 & 48.24 & 80.52 & 77.84 & 59.06 & 54.79 & 78.55 & 75.22 & 53.73 & 49.33 & 84.08 & 81.47 & 61.77 & 58.37\\
    & & IFSL & 77.03 & 75.42 & 59.07 & 55.98 & 81.50 & 78.90 & 63.47 & 59.42 & 80.15 & 76.93 & 62.99 & 59.24 & 85.48 & 82.94 & 69.16 & 66.48\\

    \rowcolor{white}
    & \multicolumn{1}{c}{\multirow{2}{*}{\shortstack{k-NN}}} & & 76.63 & 73.03 & 55.92 & 50.20 & 80.85 & 77.34 & 62.94 & 56.05 & 79.60 & 74.28 & 60.34 & 53.12 & 84.67 & 81.67 & 67.25 & 59.83\\
    \multirow{-6}{*}{\STAB{\rotatebox[origin=c]{90}{\textbf{Fine-Tune}}}} & & IFSL & 78.42 & 76.36 & 62.31 & 57.48 & 81.98 & 79.53 & 65.71 & 61.50 & 81.08 & 77.74 & 64.98 & 60.01 & 78.54 & 83.65 & 70.94 & 66.76\\
    \midrule
    
    \rowcolor{white}
    & \multicolumn{1}{c}{\multirow{2}{*}{\shortstack{MAML~\cite{finn2017model}}}} & & 70.85 & 67.90 & 56.59 & 52.19 & 74.02 & 71.27 & 59.17 & 54.77 & 73.92 & 70.65 & 58.02 & 53.03 & 77.20 & 74.19 & 61.40 & 57.37\\
    & & IFSL & 76.37 & 73.89 & 59.36 & 55.11 & 81.04 & 78.52 & 63.88 & 59.56 & 79.25 & 76.92 & 62.84 & 58.39 & 85.10 & 83.10 & 67.70 & 64.01\\

    \rowcolor{white}
    &\multicolumn{1}{c}{\multirow{2}{*}{\shortstack{LEO~\cite{rusu2018meta}}}} & & 74.49 & 71.34 & 58.48 & 53.93 & 80.25 & 77.68 & 65.59 & 61.17 & 75.86 & 72.66 & 59.77 & 54.84 & 82.15 & 79.84 & 68.90 & 64.83\\
    & & IFSL & 76.48 & 73.66 & 60.32 & 55.95 & 80.97 & 78.44 &  &  & 77.72 & 74.60 & 61.71 & 56.85 & 84.80 & 82.71 &  & \\

    \rowcolor{white}
    &\multicolumn{1}{c}{\multirow{2}{*}{\shortstack{MTL~\cite{sun2019meta}}}} & & 75.65 & 72.60 & 58.49 & 54.16 & 81.14 & 78.30 & 64.29 & 60.71 & 77.30 & 74.37 & 62.99 & 58.71 & 83.23 & 81.25 & 70.08 & 66.47\\
    & & IFSL & 78.03 & 75.70 & 61.17 & 57.02 & 82.35 & 79.05 & 65.72 & 62.18 & 80.20 & 77.63 & 64.4 & 60.20 & 86.02 & 84.51 & 71.45 & 68.10\\

    \rowcolor{white}
    &\multicolumn{1}{c}{\multirow{2}{*}{\shortstack{SIB~\cite{hu1empirical}}}} & & 78.88 & 76.89 & 67.10 & 64.09 & 85.09 & 83.24 & 77.64 & 74.29 & 81.73 & 79.48 & 71.31 & 68.32 & 88.19 & 86.43 & 81.97 & 80.09\\
    & & IFSL & 80.32 & 78.31 & 68.85 & 65.76 & 85.43 & 83.50 & 78.03 & 74.65 & 83.21 & 80.90 & 73.51 & 70.30 & 88.69 & 86.97 & 83.07 & 81.10\\

    \rowcolor{white}
    &\multicolumn{1}{c}{\multirow{2}{*}{\shortstack{MatchingNet~\cite{vinyals2016matching}}}} & & 75.21 & 72.35 & 61.05 & 56.70 & 79.92 & 77.60 & 66.01 & 62.04 &  &  &  &  &  &  &  & \\
    \parbox[t]{2mm}{\multirow{-10}{*}{\rotatebox[origin=c]{90}{\textbf{Meta-Learning}}}} & & IFSL & 76.73 & 73.94 & 62.64 & 58.40 &  &  &  &  &  &  &  &  &  &  &  & \\
    \bottomrule
\end{tabular}

==> tables/sq.tex <==
\begin{tabular}{c c c c}
    \hline
    \hline
    \textbf{n-shot} & \textbf{Adj.} & $\mathbf{\mathcal{S}\sim\mathcal{Q}}$ & $\mathbf{\mathcal{S}\not\sim\mathcal{Q}}$\\
    \hline
    \multicolumn{1}{c}{\multirow{4}{*}{$\mathbf{1}$\textbf{-shot}}} & \xmark & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{ft} & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{cl} & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{ft+cl} & \textbf{78.54} $\pm$ \textbf{0.13} & \textbf{78.54} $\pm$ \textbf{0.13}\\
    \hline
    \multicolumn{1}{c}{\multirow{4}{*}{$\mathbf{5}$\textbf{-shot}}} & \xmark & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{ft} & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{cl} & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{ft+cl} & \textbf{78.54} $\pm$ \textbf{0.13} & \textbf{78.54} $\pm$ \textbf{0.13}\\
    \hline
    \multicolumn{1}{c}{\multirow{4}{*}{$\mathbf{10}$\textbf{-shot}}} & \xmark & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{ft} & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{cl} & 78.54 $\pm$ 0.13 & 78.54 $\pm$ 0.13\\
    & \emph{ft+cl} & \textbf{78.54} $\pm$ \textbf{0.13} & \textbf{78.54} $\pm$ \textbf{0.13}\\
    \hline
    \hline
\end{tabular}

